Temporal Betweenness Centrality on Shortest Walks Variants

Betweenness centrality has been extensively studied since its introduction in 1977 as a measure of node importance in graphs. This measure has found use in various applications and has been extended to temporal graphs with time-labeled edges. Recent research by Buss et al. and Rymar et al. has shown that it is possible to compute the shortest path betweenness centrality of all nodes in a temporal graph in $O(n^3\,T^2)$ and $O(n^2\,m\,T^2)$ time, respectively, where $T$ is the maximum time, $m$ is the number of temporal edges, and $n$ is the number of nodes. These approaches considered paths that do not take into account contributions from intermediate temporal nodes. In this paper, we study the classical temporal betweenness centrality paths that we call \textit{passive} shortest paths, as well as an alternative variant that we call \textit{active} shortest paths, which takes into account contributions from all temporal nodes. We present an improved analysis of the running time of the classical algorithm for computing betweenness centrality of all nodes, reducing the time complexity to $O(n\,m\,T+ n^2\,T)$. Furthermore, for active paths, we show that the betweenness centrality can be computed in $O(n\,m\,T+ n^2\,T^2)$. We also show that our results hold for different shortest paths variants. Finally, we provide an open-source implementation of our algorithms and conduct experiments on several real-world datasets. We compare the results of the two variants on both the node and time dimensions of the temporal graph, and we also compare the temporal betweenness centrality to its static counterpart. Our experiments suggest that for the shortest foremost variant looking only at the first $10\%$ of the temporal interaction is a very good approximation for the overall top ranked nodes.

==> abstract.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../paper_discrete.tex"
%%% End:


==> sections/experimental_results.tex <==
\section{Experimental results}\label{sec:experiments}
\begin{table}[h!]
    \centering
    \begin{tabular}{l|ccc|cc|cc}
    \hline
     & nodes & events & edges  &  \multicolumn{2}{c|}{non-strict} & \multicolumn{2}{c}{strict}  \\ 
     \hline
     &  &  &   & active & passive & active & passive  \\ 
    \hline  
    primaryschool (d)& $242$ & $3100$ & $125773$ & $207.4$ & $413.7$ & $202.4$ & $399.5$\\
    highschool2012 (d) & $180$ & $11273$ & $45047$ & $280.7$ & $81.36$ & $266.8$ & $83.87$\\
    highschool2012 & $180$ & $11273$ & $45047$ & $416.5$ & $1208$ & $393.2$ & $1141$\\
    hospital (d) & $75$ & $9453$ & $32424$ & $45.84$ & $39.80$ & $45.13$ & $40.68$\\
    hospital & $75$ & $9453$ & $32424$ & $88.14$ & $583.9$ & $83.61$ & $555.2$\\
    ht09 (d) & $113$ & $5246$ & $20818$ & $52.02$ & $31.73$ & $51.52$ & $32.33$\\
    ht09& $113$ & $5246$ & $20818$ & $72.09$ & $241.4$ & $69.46$ & $230.3$\\
     workplace2013 (d) & $92$ & $7104$ & $9827$ & $41.21$ & $2.522$ & $40.32$ & $2.576$\\
     workplace2013 & $92$ & $7104$ & $9827$ & $57.05$ & $72.41$ & $56.03$ & $73.40$\\    
    \end{tabular}
    \caption{Statistics for the datasets. From left to right  number of nodes, number of event times, number of edges. The execution time in seconds of Algorithm~\ref{algo:betweenness} for shortest active, shortest passive, strict shortest active, strict shortest passive.}
    \label{tab:gen_stat}
\end{table}
For our experimentations we used a highly modified version of the code of \cite{buss2020algorithmic} which can be found online\footnote{\href{https://github.com/busyweaver/code_temporal_betweenness_}{github.com/busyweaver/code\_temporal\_betweenness\_}}. The code is written in \CC. We used an Intel(R) Xeon(R) Silver $4210R$ CPU $2.40$GHz without parallel processes. All datasets are available publicly\footnote{\href{sociopatterns.org}{sociopatterns.org}}. The (d) next to the name of a dataset signifies that edges are taken as directed. The same dataset without (d) means the edges are taken undirected. On table~\ref{tab:gen_stat}, in the last four columns we see the execution times of our implementation. We notice that our execution time on passive paths is slower than \cite{buss2020algorithmic}. There are several factors to explain it. The processor used in their experiments is $1.5$ times faster than ours. Morevoer, the authors used a stack to avoid using recursive functions in their code while we do not. Finally, our implementation on shortest paths is a more general purpose and active paths needs a predecessor graph ordering to account for them.    

\begin{table}[h!]
    \centering
    \begin{tabular}{lccc|ccc|ccc|ccc}
    \hline
        & \multicolumn{3}{c|}{act vs pas}  & \multicolumn{3}{c|}{str act vs str pas} & \multicolumn{3}{c|}{act vs str act}  & \multicolumn{3}{c}{pas vs str pas} \\
        \hline
        & all & nodes & times & all & nodes & times & all & nodes & times & all & nodes & times \\
        \hline
        primaryschool (d)& $0.97$ & $0.70$ & $0.61$ & $0.97$ & $0.70$ & $0.61$ & $0.99$ & $0.99$ & $0.99$ & $0.99$ & $0.99$ & $0.99$\\
        highschool2012 (d) & $0.99$ & $0.69$ & $0.65$ & $0.99$ & $0.69$ & $0.65$ & $0.99$ & $0.99$ & $0.99$ & $0.99$ & $0.98$ & $0.99$\\
        highschool2012& $0.98$ & $0.68$ & $0.54$ & $0.98$ & $0.68$ & $0.54$ & $0.99$ & $0.99$ & $0.99$ & $0.99$ & $0.99$ & $0.99$\\
        hospital (d)& $0.99$ & $0.84$ & $0.57$ & $0.99$ & $0.84$ & $0.57$ & $0.99$ & $1.0$ & $0.99$ & $0.99$ & $1.0$ & $0.99$\\
        hospital & $0.98$ & $0.87$ & $0.42$ & $0.98$ & $0.87$ & $0.42$ & $0.99$ & $0.99$ & $0.99$ & $0.99$ & $0.99$ & $0.99$ \\
        ht09 (d)& $0.99$ & $0.77$ & $0.68$ & $0.99$ & $0.77$ & $0.68$ & $0.99$ & $0.99$ & $0.99$ & $0.99$ & $0.99$ & $0.99$\\
        ht09 & $0.97$ & $0.76$ & $0.46$ & $0.97$ & $0.77$ & $0.46$ & $0.99$ & $0.99$ & $0.99$ & $0.99$ & $0.99$ & $0.99$\\
        workplace2013 (d)& $0.99$ & $0.76$ & $0.79$ & $0.99$ & $0.77$ & $0.79$ & $0.99$ & $0.99$ & $0.99$ & $0.99$ & $0.99$ & $0.99$\\
        workplace2013& $0.99$ & $0.72$ & $0.48$ & $0.99$ & $0.73$ & $0.48$ & $0.99$ & $0.99$ & $0.99$ & $0.99$ & $0.99$ & $0.99$\\
        % hospital & $0.98$ & $0.87$ & $0.42$ & $0.98$ & $0.87$ & $0.42$\\
        % ht09 (d) & $0.99$ & $0.77$ & $0.68$ & $0.99$ & $0.77$ & $0.68$\\
        % ht09 & $0.97$ & $0.76$ & $0.46$ & $0.97$ & $0.77$ & $0.46$\\
        % workplace2013 (d)& $0.99$ & $0.76$ & $0.79$ & $0.99$ & $0.77$ & $0.79$\\
        %       workplace2013 & $0.99$ & $0.72$ & $0.48$ & $0.99$ & $0.73$ & $0.48$\\
    \end{tabular}
    \caption{Kendall’s tau correlation pairs of rankings. From left to right : active with passive, strict active with strict passive, active with strict active, passive and strict passive. For each pairs of rankings the correlation is made on 3 rankings all: for all temporal nodes $B(v,t)$, nodes: for $B(v)$ and times: for $B(t)$.}
    \label{tab:pas_act}
\end{table}
\begin{table}[h!]
    \centering
    \begin{tabular}{lccc|ccc|ccc|ccc}
    \hline
          & \multicolumn{3}{c|}{act vs. pas} &\multicolumn{3}{c|}{str act vs. str pas} & \multicolumn{3}{c|}{act vs str act}& \multicolumn{3}{c}{pas vs str pas}\\
          \hline
                   & all & nodes & times & all & nodes & times & all & nodes & times & all & nodes & times \\
                   \hline
                   primaryschool (d)& $1$ & $3$ & $1$ & $1$ & $3$ & $1$ & $10$ & $10$ & $10$ & $10$ & $10$ & $10$\\
                   highschool2012 (d)& $3$ & $1$ & $5$ & $4$ & $1$ & $5$ & $9$ & $10$ & $10$ & $10$ & $10$ & $10$\\
                   highschool2012& $0$ & $5$ & $2$ & $0$ & $5$ & $2$ & $10$ & $10$ & $10$ & $9$ & $10$ & $8$\\
                   hospital (d) & $2$ & $8$ & $2$ & $2$ & $8$ & $2$ & $10$ & $10$ & $10$ & $10$ & $10$ & $10$\\
                   hospital & $1$ & $8$ & $1$ & $1$ & $8$ & $1$ & $10$ & $10$ & $10$ & $10$ & $9$ & $10$\\
                   ht09 (d) & $5$ & $8$ & $6$ & $5$ & $8$ & $6$ & $10$ & $10$ & $10$ & $10$ & $10$ & $10$\\
                   ht09& $2$ & $8$ & $2$ & $2$ & $8$ & $2$ & $10$ & $10$ & $10$ & $10$ & $10$ & $10$\\
                   workplace2013 (d)& $6$ & $4$ & $7$ & $6$ & $4$ & $8$ & $10$ & $10$ & $9$ & $10$ & $10$ & $10$\\
          workplace2013& $0$ & $7$ & $0$ & $0$ & $7$ & $0$ & $10$ & $10$ & $10$ & $9$ & $10$ & $10$\\
          % primaryschool (d) & $4$ & $8$ & $3$ & $8$\\
          % highschool2011 (d)& $7$ & $7$ & $8$ & $8$\\
          % highschool2011& $4$ & $4$ & $3$ & $6$\\
          % hypertext & $7$ & $9$ & $7$ & $9$\\
    \end{tabular}
    \caption{Size of the intersection for pairs rankings of the ten vertices with highest temporal betweenness values. From left to right: active with passive, strict active with strict passive, active with strict active and passive with strict passive. For each pairs of rankings the correlation is made on 3 rankings all for all: temporal nodes $B(v,t)$, nodes: for $B(v)$ and times: for $B(t)$.}
    \label{tab:inter}
\end{table}
On Table~\ref{tab:pas_act} and Table~\ref{tab:inter}, the subcolumns all, nodes and times, represent the values of betweennes centrality for respectively all temporal nodes $B(v,t)$, the overall betweenness of a node $B(v)$ and the overall betweenness of a time $B(t)$, see Equation~\ref{eq:overall}. Our main findings is that the rankings correlations of active and passive types are high if we are looking at all temporal nodes. However, the correlations are much lower if we look at the rankings of nodes or times. See first 2 subsets of 3 columns in Table~\ref{tab:pas_act} and Table~\ref{tab:inter}. 


==> sections/figs/time_table.tex <==
dataset & nodes & events & edges & agg_edges & Buss & sh pas & sh act  & sh-rl act & sh-rl pas & sh-fm pas  & static \\ 
gre & $1547$ & $1300$ & $113112$ & $3680$ & $1924.1$  & $2921.2$  & $9067.7$  & $1496.3$  & $5535.6$  & $3839.8$ & $21.156$ \\
ren & $1407$ & $10825$ & $107384$ & $3718$ & $2480.7$  & $3343.4$  & $26144$  & $1656.3$  & $22379.$  & $3329.3$ & $29.046$ \\
bel & $1917$ & $1132$ & $120951$ & $6440$ & $2530.8$  & $3512.9$  & $12691.$  & $2056.5$  & $8111.3$  & $3753.4$ & $45.057$ \\
kuo & $549$ & $1211$ & $30545$ & $1952$ & $169.45$  & $242.67$  & $683.99$  & $119.67$  & $514.47$  & $240.69$ & $1.9935$ \\
prim & $242$ & $3100$ & $125773$ & $16634$ & $1146.2$  & $1701.6$  & $454.91$  & $761.39$  & $435.49$  & $1597.1$ & $4.0661$ \\
hs11 & $126$ & $5609$ & $28539$ & $3418$ & $75.741$  & $98.333$  & $101.61$  & $40.064$  & $89.428$  & $107.29$ & $0.3405$ \\
hs12 & $180$ & $11273$ & $45047$ & $4440$ & $208.56$  & $287.82$  & $371.63$  & $142.94$  & $384.21$  & $299.61$ & $0.9211$ \\
hp & $75$ & $9453$ & $32424$ & $2278$ & $121.75$  & $170.15$  & $76.980$  & $75.908$  & $59.653$  & $177.97$ & $0.1877$ \\
ht & $113$ & $5246$ & $20818$ & $4392$ & $43.157$  & $61.687$  & $63.644$  & $34.362$  & $65.114$  & $66.632$ & $0.2166$ \\
wp & $92$ & $7104$ & $9827$ & $1510$ & $12.020$  & $16.154$  & $51.370$  & $7.4984$  & $50.847$  & $17.592$ & $0.0782$ \\

